Mosaic: Policy Homomorphic Network Extension

With the advent of large-scale cloud computing infrastructure, network extension and migration has emerged as a major challenge in the management of modern enterprise networks. Many enterprises are considering extending or relocating their network components, in whole or in part, to remote, private and public data centers, in order to attain scalability, failure resilience, and cost savings for their network applications. In this paper, we conduct a first rigorous study on the extension and migration of an enterprise network while preserving its performance and security requirements, such as layer 2/layer 3 reachability, and middle-box traversal through load balancer, intrusion detection and ACLs. We formulate this increasingly important problem, present preliminary designs, and conduct experiments to validate the feasibility of our designs.

==> conclusion.tex <==
\vspace{-0.08in}
\section{Conclusion and future work}
\label{sec:conclusions}
Network extension and migration are now a major challenge for
large-scale networks, attracting industrial attention (\eg,
~\cite{CiscoL2ext,IBMJuniperHybrid,vpn-cubed,WoodVPC09}).  Ad-hoc
methods of network extension and migration can result in serious policy
violations. In this paper, we present the first 
framework for network policy specification.  Furthermore, we evaluate the
feasibility of policy homomorphic network extension and
migration to remote data centers.


==> introduction.tex <==
\myvspace{-0.1in}
\section{Introduction} 
\label{sec:introduction}

Due to enterprise dynamics (\eg, expansion into a new site), hardware
consolidation, and the emergence of cloud computing infrastructures,
network extension and migration has become a major challenge in the 
management of modern enterprise networks. On the one hand, as many 
enterprises run out of space in their existing data 
centers~\cite{viridity}, they need to extend or relocate their network 
to new private data centers. On the other hand, recent emergence of 
public cloud computing infrastructure provides enormous opportunities 
for an enterprise to either replace or complement its existing servers 
with computing resources in the cloud, in order to take advantage of 
improved efficiency and reliability. We refer to the private or 
public data centers that an enterprise extends to as the 
{\em remote data centers}.

Despite their potential business benefits and needs, such extension 
and migration can become quite complex and pose substantial challenges
to the operation of enterprise network infrastructure. In particular, 
such extensions often have to be incremental instead of a complete
restructuring of the existing network infrastructure. Thus, a seemingly 
small extension can be extremely challenging to handle in practice.

Consider a simple example of relocating a set of application servers
from one data center of the enterprise to a remote data center (\eg,
another private or public cloud data center). These servers usually
have complex communication patterns regulated by network policies such
as traversal of firewalls and intrusion detection systems before being
reached. Furthermore, an enterprise network may enforce network
policies using a variety of techniques including routing design,
topology design, and deployment of policy boxes at strategic
locations.  Some such techniques, such as deployment at topology cuts,
can be implicit without any explicit representation.
%implicit 
Consequently, it can be extremely challenging to take these servers
out of their current ``context'' and place them into another
``context'' while preserving existing network policies. Manual
reconfiguration, although maybe feasible for small networks, can no
longer satisfy the need to scalable to large systems.
%However, such designs can be
%implicit, leading to substantial challenges in evaluating policy
%preservation during network extension. 

%the flexibility in network construction at the remote data centers. 
There are two common ways to connect an enterprise network to a 
remote data center. In one extreme, a remote data center may belong to 
the same enterprise, allowing plenty of flexibility in constructing
network topology and policy boxes inside the remote data center. 
In the other extreme, a remote data center may belong to a public cloud 
provider, imposing substantial restrictions on the connection and layout 
of the remote data center.
%available 
%techniques to connect to the remote data center and how the enterprise can construct topology and policy boxes
%inside the remote data center.

%Enterprises business and computing needs can change rapidly given the
%constant changing economic conditions and competitive landscape. This
%entails changing needs of IT resources. Cloud computing providers
%offer infrastructure as a server with a pay-as-you-go resource leasing
%model. This is a powerful model for enterprises to efficiently utilize
%IT resources when the need arises. 

%Currently start-ups have been using Amazon EC2 services with
%essentially no in-house IT infrastructure other than computers and
%networking support for accessing EC2. Large companies such as
%pharmaceutical companies have been running drug develop tests in EC2.

%Currently to make use of cloud computing resources, applications have
%to be rewritten to use cloud computing storage semantics and APIs such
%as Amazon's S3 and simpleDB. At a minimal, complicated configurations
%have to be changed to make use of cloud resources, e.g. configure
%computing resources in the cloud to access enterprise resources such
%as SQL, storage. Security policies have to be applied when accessing
%internal resources.

We present Mosaic, a first framework for network extension and migration 
while preserving enterprise network policies. Mosaic introduces two key 
notions --- way-points and scopes --- to capture network policy 
constraints during network extension. Moreover, Mosaic includes two 
simple and yet powerful primitives named proxy and mirror to implement 
network extensions with provable guarantees. Guided by the policy 
contraints and utilizing the primitives, a Mosaic extension algorithm 
computes efficient network extension strategy. We refer to policy-preserving 
network extension as {\em policy homomorphic network extension}.

% MFN 
We proceed by presenting a rigorous analysis of the requirements and
constraints of preserving policies during migration. We then evaluate
our novel network extension algorithm in a large campus network setting.  
Our preliminary results indicate that Mosaic extension algorithm performs 
far better than a naive server relocation algorithm in terms of number of
policy violations.

% We implement our algorithms and conduct preliminary evaluations in a
% large campus network setting. We show that without applying our 
% framework, a naive server relocation algorithm can lead to a large 
% number (up to 80\%) of policy violations. 

% yry: redundant, as in implementation already
%\section{Implementation} 
%
%The preceding algorithm provides the core of our system. To map the
%algorithm to implementation, we need to address a set of challenges.
%
%\subsection{Extracting Constraints}
%Although we define configuration transparency using packets,
%configuration transparency can be specified succinctly. For example, a
%set of packets can be specified by their source IP prefix, destination
%IP and port. For each VLAN, we can have all the end hosts in the VLAN
%as the set of potential receivers associated with each IP
%destination in the VLAN. Similarly we can specify waypoint set by the
%set of middleboxes that need to be traversed 
%for a set of packets. The constraints $\{\tau_i\}$ can be specified by
%constraint regular expression language.   
%
%To extract $\{ tp_i \}$ might not be a trivial task. We collect
%routing FIB, packet filters, middlebox configuration files, network
%topology. We automatically come up with an initial  $\{ tp_i \}$
%expressed succinctly using constraint language. We then allow
%enterprise customers to prune the set of constraints. 
%
%\subsection{Policy Specification}
%The specification language needs to specify middlebox traversals. 
%
%\subsection{Enterprise Network Device Reconfiguration}
%Our techniques can be readily deployed in the enterprise networks. All
%we need is the support of tunnels in IP layer, and the capability of
%filtering routes by router information base (RIB). That is, the
%control plane of the router does not install a particular
%router. These capabilities are present in existing routers.
%
%\subsection{Cloud Configuration}
%We use virtual switch (vswitch) in the hypervisor to implement
%potential receiver set. We implement logical middleboxes in hypervisor
%as well. {\bf not clear what we can do here? What to assume about
%VPC?}
%
%
%
%The rest of the paper is organized as follows. In
%Section~\ref{sec:motivation}, we give a motivating example. In
%Section~\ref{sec:policy}, we present our framework to define network
%policies for network extension. We present the Mosaic Proxy algorithm
%in Section~\ref{sec:proxy}, and the Mirror algorithm in
%Section~\ref{sec:mirror}.  In Section~\ref{sec:eval}, we evaluate the
%two algorithms. In Section~\ref{sec:opt}, we propose ways to optimize
%our two algorithms.
%% We discuss additional issues in
%% Section~\ref{sec:discussions},  and 
%We conclude in Section~\ref{sec:conclusions}.


==> overview.tex <==
\vspace{-0.08in}
\section{Mosaic Overview}
\label{sec:overview}

The motivating example reveals potential issues facing the extension
of an enterprise network into a remote data center. Mosaic is a 
systematic framework to address these issues. Mosaic consists of two 
major components: policy specification and network transformation.

%\begin{itemize}
%\item Policy specification
%\item Network transformation algorithm
%\end{itemize}

%\begin{figure}[tbp]
%\centering
%\includegraphics[width=0.48\textwidth]{figures/arch.ps} 
%\caption{Functional components of Mosaic} \label{fig:arch}
%\end{figure}

\para{Policy specification:} 
To systematically investigate and solve the problems raised in the
preceding section, we need to explicitly define the policies that an
enterprise network intends to enforce so that one can validate any 
given solution. Policies capture the ``invariants'' that network 
extension should preserve. Since network extension alters an existing 
network topology (\eg, by adding new nodes or relocating existing 
nodes), the {\em traversal} and {\em scope} of a packet (or frame if 
we talk about layer 2) can deviate from those in the original network. 
Thus, policy specification is crucial for policy enforcement, which
will be discussed in Section~\ref{sec:policy}.
%Such deviations can cause policy violations. 

\para{Network transformation:}
Bounded by policy specification, network transformation computes the 
configuration at the remote data centers as well as at the local 
enterprise network. In addition to policies, multiple other factors, 
including objectives and constraints on application performance and 
migration costs, contribute to the complexity and effectiveness of 
network transformation.

The capabilities of network devices influence what transformation 
techniques may be used. In this paper, we do not assume the 
availability of futuristic mechanisms such as pswitches~\cite{pswitch08} 
and OpenFlow~\cite{openFlow}. While these mechanisms can simplify our 
solutions, they have not been widely adopted so far. Instead, we only 
consider the traditional mechanisms that are readily available in 
today's enterprise networks. In Section~\ref{sec:algorithm}, we will
discuss the primitives and algorithmic framework of Mosaic.

%Ideally, there should be a single algorithm to conduct network
%transformation. Thus far, however, such an algorithm is
%elusive. Instead, we present algorithms for two cases on opposite
%sides of the spectrum. We emphasize that the algorithms utilize the
%common policy framework as a unifying scheme.

%Specifically, Table X below shows the combinations on the capabilities
%at the enterprise and the remote data center, as well as the effective
%algorithms.

%In this paper, we focus mainly on the settings of connecting the local
%enterprise network to the remote data center using L3
%connectivity. This is motivated by the interoperability and universal
%availability of IP connectivity. In discussions, we evaluate using L2
%connectivity, but our presentation below focuses on using L3
%connectivity.


==> policy.tex <==
\vspace{-0.1in}
\section{Policy Specification} 
\label{sec:policy}
%\subsection{Policies in Original Network}

We start with the policy specification. We represent the topology of 
the original enterprise network $G$ using $V$, the set of nodes 
consisting of end hosts (servers, virtual machines), switches, routers 
and middleboxes; and $E$, the set of connections among network nodes.  

An enterprise network operator defines policies $P$ on packets and
frames, based on topology, as we have seen in the motivating example. 
Since we treat L3 packets and L2 frames uniformly in our framework, 
we use packet as a general term. For a given packet, policies specify 
additional information beyond what is already contained in the packet.  
Specifically, for a given packet $pkt_i$, policy $\tt{Policy}_i$ 
consists of not only destination(s) $\tt{Destination}_i$ but also two 
additional perspectives: waypoints $\tt{Waypoints}_i$ and scope 
$\tt{Scope}_i$.

%erranlli-ladis:
By default, packets not associated with any policy are unwanted. These
packets must be filtered before reaching their destinations. This
default policy captures un-reachability policies which are typically
enforced by limiting route redistributions and specifying access
control lists (ACLs) in routers. 

% MFN
%The policy specification represents the first comprehensive attempt
%to organize and classify network policy in terms of its waypoints and scope.

%\subsection{Waypoints}
\para{Waypoints:}
The waypoints of a packet are the network nodes in addition to the
destination(s) that should receive the packet. An enterprise may
design its network such that a packet should pass through a particular 
set of network nodes. In the motivating example, we see that packets 
from the Internet should visit an intrusion prevention box before 
reaching a tier-1 server. As another example, an enterprise network 
may deploy a sniffer that is connected to the mirror port of a switch 
to receive a copy of a given packet for logging purpose. In this case, 
the sniffer also belongs to the waypoints of the given packet. Let 
$\tt{Waypoints}_i$ be the waypoints of packet $pkt_i$.

Waypoints are specified by using the {\em ordering} and {\em occurrence}
constraints. Ordering specifies if there are any constraints on the 
order to visit the nodes in the waypoints. For example, an enterprise 
network may require a packet to visit one middlebox before visiting 
another one. Occurrence specifies the number of times that a middlebox 
should be visited. For example, a packet may visit a middlebox only once, 
or none at all. We write $\tt{Waypoints}_i(\tt{Order_i},\tt{Occurrence_i})$ 
to emphasize that $\tt{Waypoints}_i$ requires the ordering and occurrence 
constraints for $pkt_i$. 

It is important to realize that we use network nodes in a generic 
sense when specifying waypoints. We can view each network node, in
particular, a middlebox, as the member of a function class (\eg, 
firewall, intrusion prevention, or sniffer) with a specific 
configuration state. 
%Using object-oriented terminology, we can view each network
%node as an instance of a particular function class. 
Formally, we denote the function class of the middlebox node $v_j$ as
$\tt{class}(v_j)$; and its configuration state as $\tt{conf}(v_j)$. 
%In practice, the understanding is that a
%waypoint node (for a given packet) specifies its function class
%as well as its configuration state.

As an example, consider the network in Figure~\ref{fig:mot-ex}. The
tier-1 and tier-2 firewalls have the same function class: 
$\tt{class}(F_1)$ = $\tt{class}(F_2)$ = $\tt{Firewall}$. But
their configuration states are different: the tier-1 firewall is in 
charge of the first line of defense and thus is configured to allow 
only HTTP traffic; the tier-2 firewall handles traffic from the
tier-1 servers and intranet and thus may allow more protocols.  

%Thus, if we specify that a packet from an Internet client to a tier-1
%server must traverse a tier-1 firewall; but, if the packet traverses a
%tier-2 firewall instead (without traversing tier-1 firewall), then it
%violates the policy.

% Another important component in the specification of waypoints is that
% there can be {\em ordering} and {\em occurrence} constraints. Ordering
% specifies if there are any constraints on the order to visit the nodes
% in the waypoints. For example, an enterprise network design may
% require that a packet visit one middlebox before visiting another
% one. Occurrence specifies the number of times that a middlebox can be
% visited. For example, a packet may visit a middlebox only once, or
% none at all. We write $\tt{Waypoints}_i(\tt{Order_i},
% \tt{Occurrence_i})$ when we want to emphasize that $\tt{Waypoints}_i$ 
% includes the ordering and occurrence constrains for $pkt_i$.

%\subsection{Scope}
\para{Scope:}
Destinations and waypoints capture the nodes that a packet {\em must} 
visit. However, a packet {\em may} reach other nodes in an enterprise 
network. For example, a modern switch may flood a given packet to a 
layer 2 domain if a forwarding entry is not present in its layer 2 
FIB (forwarding information base); routers and switches along the path 
from the source to the destinations will see the packet (if unencrypted); 
due to routing changes, some routers not on the normal forwarding path 
may also see the packet. 
% yry: ??
%Router ACLs on the data path and route redistribution in the control
%path will also limit the potential nodes a packet can traverse. 
We associate a \emph{scope} with each packet, which defines the 
security zone of the packet. The scope is the maximum set of nodes 
that a packet can reach. Let $\tt{Scope}_i$ be the scope of $pkt_i$.

%\subsection{Example Policies}
\para{Example Policies:}
We now illustrate the preceding concepts using the example shown in
Figure~\ref{fig:mot-ex}.  Figure~\ref{prog:sample} specifies six
policies for the network.

Policy $\tt{Policy}_1$ specifies that any HTTP request packet $pkt_1$
to a tier-1 application server from an Internet client must traverse tier-1
firewall, tier1 load balancer (the tier-1 application's public
accessible IP is configured at the load balancer $LB_1$). The packet's
destination is changed to a tier-1 server $u_1$ by $LB_1$. We treat
this as a new packet $pkt_2$. This packet
with source $u_e$ and destination $u_1$ which originates from $L_1$
needs to traverse $IPS_1$. 
%erranlli: do we need this?
%($u_e:L_1$ stands for source $u_e$ originates from $L_1$).  
The scope of $pkt_1$ $\tt{Scope}_1=\{LB_1,$ $F_1, CE, S_1,
u_e\}$. The scope of $pkt_2$ $\tt{Scope}_2=\{LB_1, IPS_1,S_3, u_1\}$.

Policy $\tt{Policy}_3$ says that, any reply packet $pkt_3$ from a
tier-1 server to an Internet client must be sent to the load balancer
first. It should be checked by $IPS_1$. 

Policy $\tt{Policy}_4$ says that, for any packet $pkt_4$ with source
$LB_1$ originating from $u_1$, destined to an Internet client needs no
further checks. $\tt{Scope}_3=\tt{Scope}_2$ and
$\tt{Scope}_4=\tt{Scope}_1$. 

Policy $\tt{Policy}_5$ states that a tier-1 server's packet $pkt_5$ must
traverse tier-2 firewall and load balancer $LB_2$.  The scope
$\tt{Scope}_5=\{u_1, u_2, F_2, LB_2, IPS_2,$ 
$S_1, S_2, S_3, S_4, IPS_1, LB_1\}$. 

Policy $\tt{Policy}_6$ states that cross-traffic between tier-1 servers in
different subnet must be checked by $IPS_1$. The scope
$\tt{Scope}_6= \{u_1, v_1, IPS_1, S_3\}$. 

%erranlli: I do not know how you want to represent Order and Occurence todo
\program{prog:sample}
    {Policies for enterprise network in Figure~\ref{fig:mot-ex}.}
{\\
// 1. Internet client $u_e$ to a tier-1 application \\
$\tt{Policy}_1= ([u_e, L_1, *, 80, TCP], \tt{Scope}_1,
    \tt{Waypoints}_1(\{F_1LB_1\},$ \\
\>\>\>\>\> $\{ \sigma \vert \tt{Ocurr}(\sigma, F_1)=1, \tt{Ocurr}(\sigma, LB_1)=1\}) $\\
$\tt{Policy}_2= ([u_e, u_1, *, 80, TCP], \tt{Scope}_2,
    \tt{Waypoints}_2(\{IPS_1\},$ \\
\>\>\>\>\> $\{\sigma \vert \tt{Ocurr}(\sigma,  IPS_1)>0 \}) $\\
\\

// 2. Tier-1 application server $u_1$'s reply to Internet client $u_e$ \\ 
$\tt{Policy}_3= ([u_1, u_e, 80, *, TCP], \tt{Scope}_3, $ \\ 
\>\>\>\>\>  $\{ \sigma \vert \tt{Ocurr}(\sigma, LB_1)=1,\tt{Ocurr}(\sigma, IPS_1)>0\}) $\\
$\tt{Policy}_4= ([u_1, u_e, 80, *, TCP], \tt{Scope}_4,  \tt{Waypoints}_2(
    \{ \},\{\})) $\\
\\

// 3. Tier-1 application server $u_1$ communicates with tier-2 server $u_2$ \\
$\tt{Policy}_5= ([u_1, u_2, *, *, TCP], \tt{Scope}_5, \{ F_2 LB_2
IPS_2 \},$ \\
\>\>\>\>\>  $  \{ \sigma \vert \tt{Ocurr}(\sigma, F_2)=1, \tt{Ocurr}(\sigma,LB_2)=1,
\tt{Ocurr}(\sigma, IPS_2)>0\} ) $\\
\\

// 4. Tier-1 application server $u_1$ in subnet 1 communicates with tier-1 \\
// ~~application server $v_1$ in subnet 2 \\
 $\tt{Policy}_6= ([u_1, v_1, *, *, TCP], \tt{Scope}_6, \tt{Waypoints}_6(\{IPS_2\},$ \\
\>\>\>\>\> $\{\sigma \vert \tt{Ocurr}(\sigma,  IPS_2)>0 \}) $\\
}

%\subsection{\PH}
%With the preceding introduction on policies, we can now define \ph\
%for a given enterprise network $G(V, E, P=\{\tt{Policy}_i\})$, where
%$P=\{\tt{Policy}_i\}$ is the set of policies defined for the original
%enterprise network.
%
%We focus on the case of relocating the set $U$ of end points to the
%remote data center, say placed behind a node $v_{target}$ at the
%remote data center. We say that the objective of network extension is
%to reconnect $U$ below $v_{target}$.
%
%Let the new network be $G'(V', E',$ $\{\tt{Policy}'_i\})$. Since a
%$pkt_i$ to a host in $U$ will traverse nodes in the remote network, we
%need to extend $Scope'_i$ to include nodes it is allowed to traverse
%in the remote network. $\tt{Waypoints_i}$ is equivalent to
%$\tt{Waypoints}'_i$ iff, for each waypoint $v_j$ in
%$\tt{Waypoints}_i$, there is a corresponding waypoint $v'_j$ in
%$\tt{Waypoints}'_i$ such that $class(v_j)=class(v'_j)$ and
%$conf(v_j)=conf(v'_j)$. 
%
%The two networks $G$ and $G'$ are \phic \ iff each policy
%$\tt{Policy}_i$ is waypoints equivalent to $\tt{Policy}'_i$ and the
%packet $pkt_i$ can not go out of the extended $Scope'_i$.



==> related.tex <==
\section{Related work} 
There are two main bodies of related work. The first one is on creating
virtual private resources for public data centers. The second one is
on enterprise network design and access control. 

\para{Virtual private resources for public data centers:}
Virtual private connection can be done in L2, L3 and
overlay. CloudNet~\cite{WoodVPC09} enables an enterprise to extend its
VLANs seamlessly into public data centers. CloudNet makes use of ISP
provisioned VPLS service. Cisco~\cite{CiscoL2ext} discusses various
technologies that can enable L2 extension of enterprise network to
remote data centers. IBM and Juniper Networks~\cite{IBMJuniperHybrid}
have demonstrated how a hybrid cloud could allow enterprises to
seamlessly extend their private clouds to remote servers in a secure
public cloud. However, there are not much detail given.

Amazon VPC~\cite{amazon-vpc} provides seamless integration of cloud
resources with enterprise sites in the IP layer. It does not need ISP
support. It sets up IPSec tunnels between a customer edge router and
the Amazon VPC gateway. BGP route announcements are setup between the
two routers.  VPN-Cubed~\cite{vpn-cubed} is a commercial product and
is an overlay solution. Virtual machines create VPN tunnels to
VPN-Cubed Manager (virtual switch). VPN-Cubed Manager routes among
virtual machines participating in overlay networks. Because it relies
on overlay routing, its performance is significantly worse than layer
2 and layer 3 VPN. However, none of these work consider \ph\ when the
network is extended.

\para{Enterprise network design and access control:}
There are recent papers on enterprise network design, reachability
analysis, access control and management~(\eg, \cite{ReachabRexford05,
sysDesignMaltz08,complexAkella09,ResonanceFeamster09, TheoIMC09}). Xie
\etal ~\cite{ReachabRexford05} formally define potential reachability
of a network. Their model unifies packet filters and routing
protocols. Benson, Akella and Maltz~\cite{TheoIMC09} define a policy
unit concept, which is an abstract representation of how the
reachability policies implemented in a network apply to different
network hosts. However, this reachability analysis does not consider
middlebox traversal policies. Sung \etal ~\cite{sysDesignMaltz08}
take a systematic design approach to optimize virtual local area
networks (VLANs) and reachability control design for enterprise
networks. Specifically, they design algorithms to optimize the group
of hosts into VLANs, placement of routers and bridges, and placement
of ACLs.  Benson, Akella and Maltz~\cite{complexAkella09} develop a
suite of complexity models that describe the routing design and
configuration of a network in a succinct fashion. The model captures
the difficulty of configuring control and data plane behaviors on
routers. Nayak \etal ~\cite{ResonanceFeamster09} introduce a new
framework for specifying dynamic access control policies for
enterprise networks, and show how it might be implemented in an
OpenFlow-based architecture. However, this work does not consider
\ph\ when the enterprise networks are extended to public or private
data centers.

There are also studies on how to deal with middleboxes in
networks~\cite{middleboxNharm04,emeFrancis07,pswitch08}.  Walfish
\etal ~\cite{middleboxNharm04} propose an extension to the Internet
architecture that facilitates the deployment of middleboxes. The new
architecture requires a set of references to be carried in packets and
serve as persistent host identifiers. It provides a way to resolve
these references to delegates chosen by the referenced host.  Guha and
Francis~\cite{emeFrancis07} present a new architecture which couples
overlay signaling with data-path signaling. The new architecture
allows a wide range of "end-middle-end" network requirements,
including access control and middlebox steering.  Joseph, Tavakoli and
Stoica~\cite{pswitch08} present an elegant approach such that
unmodified middleboxes are placed on the network path by plugging them
into \emph{pswitches}. Based on policies specified by administrators,
pswitches explicitly forward different types of traffic through
different sequences of middleboxes.  However, they do not consider how
to enforce middlebox traversal policies when networks are extended
into public or private data centers. In addition, they all change the
current architecture.

Other related work is data center networking~\cite{VL2Greenberg09,
Portland09, SEATTLE08}. The structure of data center networks can have
implications on network extensions.


\iffalse
There are papers on how to deal with middleboxes in
networks~\cite{middleboxNharm04,emeFrancis07}. There are also recent
papers on enterprise network design, access control and
management~\cite{sysDesignMaltz08,complexAkella09,ResonanceFeamster09}.
Reachability analysis~\cite{ReachabRexford05} is also relevant.  Other
related work are data center networking~\cite{VL2Greenberg09,
Portland09, SEATTLE08}. The idea of separating location address from
actual address has been applied in these data center networking
papers. However, they do not support transparent and secure cloud
resources for enterprises.

The most closely related work to ours is cloudNet~\cite{WoodVPC09},
VPN-Cubed~\cite{vpn-cubed} and Amazon virtual private cloud
(VPC). CloudNet has serious scalability in terms of the number of
virtual private clouds (VPCs) or enterprises it can support. Without
VLAN stacking, it can only support 4096 VLANs. It is not clear how to
make use of VLAN stacking to support more customers.
%It only uses VLANs to separate different customers. It does not support
%the seamless VLAN extensions of customers; that is, the cloud
%resources can belong to different VLANs of the enterprise. Servers
%within the same VLANs (but some can be in the enterprise and some in
%the cloud) should be allowed to talk to each other without being aware
%of their physical locations. It does not seem to support overlapping
%private addresses in the cloud for different enterprises. In addition,
Cloud resources such as VMs can be ephemeral, this creates significant
signaling burden in terms of switch configuration for VLANs.

VPN-Cubed is a commercial product and is an overlay solution. Virtual
machines create VPN tunnel to VPN-Cubed Manager (virtual
switch). VPN-Cubed Manager routes among virtual machines participating
in overlay networks. Because it relies on overlay routing, its
performance is significantly worse than layer 2 and layer 3 VPN. In
addition, there is no express way to connect enterprise sites with
cloud resources.

Amazon VPC seamless integrates cloud resources with enterprise sites
in the IP layer. It has no network provider support. In contrast,
Smosaic provides a layer 2 abstraction and simplifies enterprise
management of cloud resources by providing the familiar VLAN
abstraction.

IBM and Juniper Networks will demonstrate how a hybrid cloud could
allow enterprises to seamlessly extend their private clouds to remote
servers in a secure public cloud, as high priority applications are
given preference over the lower priority ones when resources become
constrained... Once installed, IBM and Juniper could seamlessly roll
client workloads from Beijing to Silicon Valley to Sao Paulo to ensure
that clients never miss a service level agreement.

Arista

L2 extension by Cisco. But their context is the simple case where
there are no middleboxes in L2 domain.

One class of related is to provide hybrid cloud in virtual
machine. Extreme proposes that switches become "VM aware." Extreme
currently supports VMware's hypervisors with plans to add others to
the mix. This will allow the company's switches to dynamically track
and manage VMs and apply policies as VMs move across the network.
%http://www.goodgearguide.com.au/article/328606/extreme\_unveils\_switching\_blueprint\_virtual\_data\_centers

Today, vendors such as Cisco and even the leading blade server
companies -- IBM, HP and Dell -- propose adding a software-based
virtual switch to the server itself to handle the growing number of
VMs. Cisco's instantiation of this is VN-Link and the Nexus 1000V
software-based switch.

But virtual soft switches on servers add another element and layer of
management complexity to the virtual data center, Extreme
asserts. Meanwhile, moving -- or keeping -- switching in the network
reduces management complexity while increasing switching performance,
the company says. So Extreme proposes keeping switching in the switch
and not moving it to the server.
\fi
